The Scope of In-Context Learning for the Extraction of Medical Temporal Constraints

Medications often impose temporal constraints on everyday patient activity. Violations of such medical temporal constraints (MTCs) lead to a lack of treatment adherence, in addition to poor health outcomes and increased healthcare expenses. These MTCs are found in drug usage guidelines (DUGs) in both patient education materials and clinical texts. Computationally representing MTCs in DUGs will advance patient-centric healthcare applications by helping to define safe patient activity patterns. We define a novel taxonomy of MTCs found in DUGs and develop a novel context-free grammar (CFG) based model to computationally represent MTCs from unstructured DUGs. Additionally, we release three new datasets with a combined total of N = 836 DUGs labeled with normalized MTCs. We develop an in-context learning (ICL) solution for automatically extracting and normalizing MTCs found in DUGs, achieving an average F1 score of 0.62 across all datasets. Finally, we rigorously investigate ICL model performance against a baseline model, across datasets and MTC types, and through in-depth error analysis.

==> bib.tex <==
\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}

==> tables/icl_prompts.tex <==
\begin{table*}[!h]
\centering 
\caption{Prompts for the \textit{simple}, \textit{guided}, and \textit{specialized} models. While there are 6 prompts for the \textit{specialized} model, we provide only the imprecise dependency (MTC Type 4) prompt for simplicity.}


\begin{tabular}{|c|c|}
\hline
\thead{Model} & \thead{Example Prompt} \\
\hline
\makecell{\textit{Simple}} & 
\makecell{Extract the medical temporal constraints from the following drug usage guideline.} \\
\hline
\makecell{\textit{Guided}} & 
\makecell{Extract the medical temporal constraints from the following drug usage guideline. \\ Use the medical temporal constraint format as defined by the context free grammar \\ below, and pay attention to the examples. \\ The context free grammar contains the following set of terminals ... \\ ... Using these terminals, medical temporal constraints can be expressed using \\ the following nonterminals ... \\ ... Normalize all activities, if similar enough, into the following list of activities: ... } \\
\hline
\makecell{\textit{Specialized}} & 
\makecell{Extract all imprecise dependency medical temporal constraints from the following samples. \\ An imprecise dependency medical temporal constraint is any instruction to take medication \\ before, while, or after another activity. MTCs are of the form X\_Y, where X is one of \\ \{before, after, while\}, and Y is an activity.} \\
\hline
\end{tabular}
\label{tab:icl_prompts}
\end{table*}

==> tables/mtc_types_dist.tex <==
\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
Dataset &Total # MTCs &MTC Type 1 &MTC Type 2 &MTC Type 3 &MTC Type 4 &MTC Type 5 &MTC Type 6 &MTC Type 7 \\
\hline
DUG Dataset &147 &17.01\% &11.56\% &1.36\% &20.41\% &0.68\% &30.61\% &18.37\% \\
\hline
FDA Dataset &560 &10.71\% &35.36\% &28.75\% &20.54\% &0.00\% &0.00\% &4.64\% \\
\hline
\end{tabular}
\label{table:mtc_types_dist}
\end{center}
\end{table}
